Transformer based Fingerprint Feature Extraction

Fingerprint feature extraction is a task that is solved using either a global or a local representation. State-of-the-art global approaches use heavy deep learning models to process the full fingerprint image at once, which makes the corresponding approach memory intensive. On the other hand, local approaches involve minutiae based patch extraction, multiple feature extraction steps and an expensive matching stage, which make the corresponding approach time intensive. However, both these approaches provide useful and sometimes exclusive insights for solving the problem. Using both approaches together for extracting fingerprint representations is semantically useful but quite inefficient. Our convolutional transformer based approach with an in-built minutiae extractor provides a time and memory efficient solution to extract a global as well as a local representation of the fingerprint. The use of these representations along with a smart matching process gives us state-of-the-art performance across multiple databases. The project page can be found at https://saraansh1999.github.io/global-plus-local-fp-transformer.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> bib.tex <==
% \begin{thebibliography}{1}



% \bibitem{IEEEhowto:kopka}
% H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%   0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

% \end{thebibliography}



==> rebuttal.tex <==
\section*{Author's Response}
We thank the reviewers for their thoughtful comments and their encouragement of our work. The major changes incorporated in the paper have been highlighted in blue. These along with some other minor changes and our responses are described as follows.
\\
\subsection{Response to Associate Editor} 
\textbf{\textit{The parallel use of local and global features has been
encouraged. There is a room for adding further experiments
and testing the generalization capability of the model. The
paper should be proof-read for grammatical errors and
typos.}}
\begin{itemize}
    \item New experimentation has been added in Sections 
    \ref{sec:score_norm} and \ref{sec:amt_local_info} to provide further insights into the combination of global and local features for fingerprint matching. Additional qualitative experimentation has been added in Section \ref{sec:intro} to demonstrate the motivation of our work.
    \item The generalization capability of the approach has been tested in Section \ref{sec:generalization}.
    \item Grammatical errors and typos have been corrected.
\\
\end{itemize}

\subsection{Response to Reviewer ID 3523}
\begin{enumerate}
    \item \textbf{\textit{Motivation. The core problem of the global approach [4]
and local approach [10] should be further analyzed in
paragraph 5 of the Introduction. The authors should focus
on the core problem of global and local approaches, which
is the motivation of the proposed method.}}
\\
In response to the comment we have expanded further on the issues pertaining to global and local approaches. This is achieved by adding a qualitative discussion of the mutually exclusive failure cases of both approaches in the Introduction(Section \ref{sec:intro}). This is followed by the enumeration of time and memory disadvantages of these approaches. The quantitative results supporting these claims have been presented in Sections \ref{sec:matching} and \ref{section:time_and_mem}.
    \\
    \item \textbf{\textit{Methodology. The method description should be improved.
Using the transformer for fingerprint feature extraction is
not the main innovation. The authors should focus on the
combination of global and local features. Moreover, the
model is constructed to solve the core problem in paragraph
6 of the Introduction, not because of the power of previous
models.}} 
    \begin{itemize}
        \item Section \ref{sec:inference} has been edited to present a more verbose description of Algorithm \ref{alg:inference} to shed more light on the combination of global and local features.
        \item A discussion about the score normalization techniques\cite{JAIN20052270} has also been added in Section \ref{sec:inference} to provide deeper insight into the combination process.
        \item An ablation study discussing the effects of different score normalization and fusion techniques has been added as Section \ref{sec:score_norm}.
        \item An ablation study discussing the effect of changing the amount of semantic local information during the combination of global and local features has been added as Section \ref{sec:amt_local_info}.
        \item Kindly note that Figure \ref{fig:scores} visualising the score distributions before and after fusing global and local scores also presents a qualitative insight into the combination process.
        \item Kindly note that Section \ref{inference_parameters} experiments with the smart combination of global and local scores using a Thresholding mechanism.
        \item Indeed such a transformer based approach has been used in other domains, but it is important to note that we are able to parallelize the global and local feature extraction only because of the architectural advantages provided by the transformer. Hence we wish to include those details in our work, but in response to the comment we have edited Sections \ref{sec:arch} and \ref{sec:train} to be more succinct.
        \\
    \end{itemize}
    \item \textbf{\textit{Experiments. The authors combine many datasets as a
dataset for experiments, which can not prove the proposed
method is effective on each dataset. More experiments
should be conducted to verify its generalization ability.}}
    \begin{itemize}
        \item As suggested in the comment we have added experimentation in Section \ref{sec:generalization} to establish the generalization capability of our approach.
        \item Kindly note that our models have been evaluated independently on each FVC sensor. The Average metrics reported are the averages of independent metrics and not a single metric on a combined test set.
        \item In response to the comment, we have now made use of a single in-house dataset as described in Section \ref{sec:data} to train and validate our models. Just like the previously used data, this too contains only optical images, but now they all come from the same source. Since the in-house dataset is quite large, we also observe a boost in performance.
        \item Since the previously used datasets are publicly available, we will retain the details of a model trained using them in the supplementary. This is done because the motivation for using public data was to make our work reproducible.
        \item Another general update was made to present $FRR@FAR=0.1\%$ in most of the experiments to keep the inferences consistent with other literature as it is a more popular metric.
        \\
    \end{itemize}
    \item \textbf{\textit{English. Many long sentences should be separated for
better understanding, and punctuation should be
appropriately added. The dash should be appropriately
added, such as "state-of-the-art" and "end-to-end," not
"state of the art" and "end to end." Some typo errors
should be corrected, such as "parallelly," not "parallely." }}
\\
Fixed.
    \\\\
\end{enumerate}

\subsection{Response to Reviewer ID 17773}
\begin{enumerate}
    \item \textbf{\textit{The authors should mention the limitations of the model and
also should mention the future research directions.}}
    \begin{itemize}
        \item Limitation of a constant number of minutiae has been added in Section \ref{sec:conclusion}.
        \item We have also added a qualitative representation of this limitation in Figure \ref{fig:mnt}.
        \item Limitations leading to vulnerabilities have also been added in Section \ref{sec:conclusion}.
    \\
    \end{itemize}
    
    
    \item \textbf{\textit{Vulnerable attacks could have been added in the
introduction and how your model is sophisticated against
those attacks.}}
    \\
    The vulnerability of spoof attacks has been recognized by us and we have already incorporated ideas from \cite{popli2021unified} to make our method resistant to them. This ongoing work has already obtained state-of-the-art results on both matching and spoof detection. But we feel like this aspect warrants a deeper discussion to do justice to its nuances, and hence we are working on another publication regarding the same.
\\\\
\end{enumerate}


